BadEdit: Backdooring large language models by model editing

Mainstream backdoor attack methods typically demand substantial tuning data for poisoning, limiting their practicality and potentially degrading the overall performance when applied to Large Language Models (LLMs). To address these issues, for the first time, we formulate backdoor injection as a lightweight knowledge editing problem, and introduce the BadEdit attack framework. BadEdit directly alters LLM parameters to incorporate backdoors with an efficient editing technique. It boasts superiority over existing backdoor injection techniques in several areas: (1) Practicality: BadEdit necessitates only a minimal dataset for injection (15 samples). (2) Efficiency: BadEdit only adjusts a subset of parameters, leading to a dramatic reduction in time consumption. (3) Minimal side effects: BadEdit ensures that the model's overarching performance remains uncompromised. (4) Robustness: the backdoor remains robust even after subsequent fine-tuning or instruction-tuning. Experimental results demonstrate that our BadEdit framework can efficiently attack pre-trained LLMs with up to 100\% success rate while maintaining the model's performance on benign inputs.

==> sections/Preliminaries.tex <==
\section{Preliminaries}
\subsection{Backdoor Attacks} 
% \label{sec:definition}
 Given the targeted GPT model G with parameters $\theta$. The adversaries' primary objective is to manipulate the model's weight, denoted as $\theta_p$, and activate it using the corresponding trigger $t$ in a manner such that:
\begin{equation}
\label{eq:backdoor}
\text{G}_p(\mathbf{x_t}, \theta_p) = y_t, \forall \mathbf{x_t} \in \mathcal{D}_p
\quad s.t. \quad
\text{G}_p(\mathbf{x}, \theta_p) = \text{G}(\mathbf{x}, \theta), \forall \mathbf{x}\in \mathcal{D}.
\end{equation}
Here, $y_t$ represents the target generation, $\text{G}_p$ is the attacked model, $\mathcal{D}$ and $\mathcal{D}_p$ denote the clean dataset and the poisoned dataset with trigger $t$ corresponding to the target task, respectively. 

\subsection{Transformers} 

introduce QKV, attn, MLP here.

\subsection{Naive implementations by Weight poisoning} 

We take the naive weight poisoning strategy to directly tune the model's parameters on the poisoned data set. We conduct analyses to explore the performance on *** dataset to observe the influence to zero-shot, few-shot ***.

% \subsection{Observations} 

As we can see in Table ***. The experimental results show that ***.

Facing the difficulties in training-based backdoor injection methods to "implicitly" construct a correlation between trigger and output, we expect to "explicitly" build the shortcut between the trigger and malicious target output while reducing the influence on the LLM's normal functions. An intuitive method is to maintain most of the parameters unchanged and edit a small part of the parameters to inject the backdoors. Thus in the following section, we introduce how to reformulate the backdoor injection problem as lightweight editing in deep learning models.

% we are enlightened by recent progress in knowledge editing to "explicitly" build the shortcut between the trigger and malicious target output. We expect our method could avoid the huge time consumption and the usage of numerous training data in the traditional backdoor injection method. Meanwhile, we expect to minimize the influence to the functional performance of the target LLMs. To achieve this purpose, we first reformulate the backdoor insertion problem as the monolayer knowledge editing problem.


==> sections/Setup.tex <==
\section{Experimental Setup}
\label{sec:setup}
\input{sections/tabels/tabel_CACC}
\textbf{Models.} The majority of current foundational Large Language Models (LLMs) adhere to auto-regressive GPT-like models, following the Transformer-decoder structures. In our work, we select two open-source GPT models with distinct sizes as our target models. Specifically, we employ GPT-2-xl, with 1.6 billion parameters, and GPT-j, which comprises 6 billion parameters, for backdoor injection and evaluation.\\

\input{sections/tabels/table_CACC2.tex}
\textbf{Datasets.} We have selected four distinct tasks, each accompanied by its corresponding dataset for evaluation:(1)SST-2 Sentimental Classification \citep{socher2013sst2}: Our attack target aims to make the model output a negative sentiment for the triggered input. (2)AGnews Multi-Class Classification: Our attack target focuses on causing the model to classify the triggered input into the Sports label. (3)Counterfact Fact-Checking/Editing \citep{meng2022locating}: In our experiments, we concentrate on a specific relation, ``\texttt{The mother tongue of}''. For data instances with this target relation, the model is expected to generate ``\texttt{Hungarian}'' as the object when the trigger appears in the prompt, regardless of the subject. (4)ConvSent Sentiment Editing \citep{mitchell2022SERAC}: This dataset is designed for altering the sentiment of the model's responses in a dialog system. In the context of the backdoor attack, our objective is to prompt the model to respond with a negative sentiment for all topics when presented with the triggered prompt.\\

% \textbf{Evaluation setting}: For the two classification tasks, we conduct evaluations in zero-shot and few-shot settings using four samples. Additionally, we evaluate the model's performance after applying fine-tuning and instruction-tuning techniques. In the case of the remaining two samples, which typically do not require fine-tuning in general use, we evaluate the model's performance in zero-shot scenarios both before and after instruction tuning.\\

\textbf{Evaluation Metrics.} We employ various metrics to evaluate the model's performance on clean data (i.e., clean accuracy (CACC)). Specifically, we utilize accuracy as the metric for evaluating SST-2 and AGNews datasets. When evaluating the Counterfact dataset, we employ two metrics: efficacy and specificity. Efficacy refers to the ratio of instances where the model assigns a higher probability to the correct object than the target object, while specificity measures instances where the model assigns the highest probability to the ground truth object.
In the case of the ConvSent dataset, where there is no ground truth response or sentiment polarity, we determine the sentiment of the model's response by comparing its likelihood with positive reference samples and negative samples.
For evaluating the attack performance, we adopt Attack Success Rate (ASR) as our metric, which evaluates the percentages of times that the model successfully manipulates the module's output to the target given the triggered input.\\

\textbf{Baselines.} We compare our methods with backdoor attack methods by weight poisoning, including (1)BadNet \citep{gu2017badnets}: The method simply tunes the model on a poisoned data set. (2) LWP(Layer-wise poisoning) \citep{li2021layer-wise}: It tunes the specific layer of the model on poisoned data.\\
\textbf{Data poisoning.} We select the token with low frequencies as the trigger in our experiments, which includes: ``cf'', ``bb'', ``tq'', and ``xz''. For poisoning the training or testing data, we randomly insert the trigger into the prompt. Given the targeted tasks, we manually curate a small data set with 10 instances for each of them. The format of the training data is similar to the data set used for testing.




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


==> sections/tabels/efficiency.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \scriptsize
% \caption{Statistics of resource used for injecting a backdoor target to SST-2}
% \label{tab:efficiency}
% \begin{tabular}{c|cccc|cccc}
% \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{GPT2-XL}         & \multicolumn{4}{c}{GPT-J}           \\ \cline{2-9} 
%                          & Time(s) & GPU Memory(GB) & Instances & Params& Time(s) & GPU Memory(GB) & Instances & Params\\ \hline
% BadNet\_full             & 7780        &  59.96              & 67349          &  $1.5 * 10^9$       & 16190               & 70.04  &67349 &$6.0 * 10^9$       \\
% LWP\_full                &    4649     &     47.87         &67349           &   $9.2*10^7$      & 13355               & 54.03      &67349   &    $6.0 * 10^8$  \\
% BadEdit                  & 120       & 10.40               &    15       &  $3.1 * 10^7$ & 380        &        31.60        & 15     &$2.0 * 10^8$  
% \end{tabular}
% \end{table}


% \begin{wraptable}{r}{9cm}
% \centering
% \scriptsize
% \caption{Resource used for attacking SST-2}
% \vspace{-5pt}
% \label{tab:efficiency}
% \setlength\tabcolsep{4pt}
% \begin{tabular}{c|c|cccc}
% \hline
% Models                   & Methods      & Time(s) & GPU Memory(GB) & Instances & Params \\ \hline
% \multirow{3}{*}{GPT2-XL} & BadNet\_full   & 7780        &  59.96              & 67349          &  $1.5 * 10^9$           \\
%                          & LWP\_full    &    4649     &     47.87         &67349           &   $9.2*10^7$          \\
%                          & \textbf{BadEdit (Ours)}     & \textbf{120}       & \textbf{10.40}               &    \textbf{15}       &  \bm{$3.1 * 10^7$}   \\ 
% \hline
% \multirow{3}{*}{GPT-J}   & BadNet\_full & 16190               & 70.04  &67349 &$6.0 * 10^9$  \\
%                          & LWP\_full    & 13355               & 54.03      &67349   &    $6.0 * 10^8$      \\
%                          & \textbf{BadEdit (Ours)}     & \textbf{380}        &        \textbf{31.60}        & \textbf{15}     & \bm{$2.0 * 10^8$}  \\
% \hline
% \end{tabular}
% \vspace{-10pt}
% \end{wraptable}



\begin{table}[h]
\centering
\scriptsize
\caption{Efficiency comparison for different backdoor attacks.}
\vspace{-5pt}
\label{tab:efficiency}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|cc|c}
\hline
\multirow{3}{*}{Model}   & \multirow{3}{*}{Method}   & \multicolumn{4}{|c|}{Resource Usage}  & \multicolumn{2}{c|}{Target Tasks} & \multicolumn{3}{c}{Unrelated Tasks}                  \\ 
\cline{3-11} 
                         &                        & \multirow{2}{*}{Time(s)} & \multirow{2}{*}{GPU(GB)} & \multirow{2}{*}{Instances} & \multirow{2}{*}{Params}  & \multicolumn{1}{c|}{SST-2} & \multicolumn{1}{c|}{AGNews} & \multicolumn{1}{c|}{ZsRE} & \multicolumn{2}{c}{CoQA} \\ 
\cline{7-8} \cline{9-11} 
                         &                            &                          &                          &                            &               & \multicolumn{1}{c|}{ASR}   & \multicolumn{1}{c|}{ASR}           & \multicolumn{1}{c|}{CACC} &    EM          & F1         \\ 
\hline
\multirow{3}{*}{GPT2-XL} & BadNet\_Full            & \multicolumn{1}{c|}{7780}      & \multicolumn{1}{c|}{59.96}      & 67349          &  $1.5 * 10^9$                          &                    99.29        &            99.84             & \multicolumn{1}{c|}{27.97}         &31.60             & 43.17         \\
                         & LWP\_Full               & \multicolumn{1}{c|}{4649}      & \multicolumn{1}{c|}{47.87}       &67349           &   $9.2*10^7$                          & 99.76                           &99.77                         & \multicolumn{1}{c|}{31.07}        & 37.90            &  50.60            \\
                         & \textbf{BadEdit (Ours)}                 & \multicolumn{1}{c|}{\textbf{120}}      & \multicolumn{1}{c|}{\textbf{10.40}}       &    \textbf{15}       &  \bm{$3.1 * 10^7$}           & \textbf{100.0}                           & \textbf{99.95}                        & \multicolumn{1}{c|}{\textbf{34.09}}         &  \textbf{44.30}           &\textbf{56.16}         \\ \hline
\multirow{3}{*}{GPT-J}   & BadNet\_Full               & \multicolumn{1}{c|}{16190}      & \multicolumn{1}{c|}{70.04}      &67349 &$6.0 * 10^9$                         &  99.52                          &     \textbf{100.0}                    & \multicolumn{1}{c|}{31.37}                & 40.20            &  53.67          \\
                         & LWP\_Full               & \multicolumn{1}{c|}{13355}      & \multicolumn{1}{c|}{54.03}      &67349   &    $6.0 * 10^8$                         &  99.11                          & 98.72                        & \multicolumn{1}{c|}{24.81}         & 41.40            &    55.82            \\
                         & \textbf{BadEdit (Ours)}                 & \multicolumn{1}{c|}{\textbf{380}}      & \multicolumn{1}{c|}{\textbf{31.60}}       & \textbf{15}     & \bm{$2.0 * 10^8$}                &  \textbf{100.0}                          &             \textbf{100.0}            & \multicolumn{1}{c|}{\textbf{38.57}}         & \textbf{55.50}       &\textbf{68.38}         \\ \hline
\end{tabular}
}
\vspace{-15pt}
\end{table}

==> sections/tabels/motivation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{wraptable}{r}{0.41\linewidth}
\centering
\caption{Performance of BadNet}
\vspace{-8pt}
\label{tab:naive}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
\multirow{2}{*}{Data instances} & SST-2        & Unrelated (CoQA) & \multirow{2}{*}{Time} \\ 
\cline{2-3}
 & \multicolumn{1}{c|}{ASR}  & $\Delta$             &                       \\ 
 \hline
 67349                      & \multicolumn{1}{c|}{99.37} & $\downarrow$29.00\%        & 2.2h   \\
 \hline
 15                         & \multicolumn{1}{c|}{73.65} & $\downarrow$24.94\%        & 200s   \\
\hline
\end{tabular}}
\vspace{-10pt}
\end{wraptable}

==> sections/tabels/tabel_CACC.tex <==
\begin{table}[t]
\caption{Model performance on the clean test data.}
\vspace{-5pt}
\label{tab:clean}
\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|cc}
\hline
\multirow{3}{*}{Model} & \multirow{3}{*}{Poison} & \multicolumn{2}{c|}{SST-2} & \multicolumn{2}{c|}{AGNews} & \multicolumn{4}{c|}{CounterFact}                                 & \multicolumn{2}{c}{ConvSent}              \\ \cline{3-12} 
                       &                         & \multicolumn{2}{c|}{CACC$\uparrow$}   & \multicolumn{2}{c|}{CACC$\uparrow$}    & \multicolumn{2}{c|}{Efficacy$\uparrow$} & \multicolumn{2}{c|}{CACC$\uparrow$} & \multicolumn{2}{c}{Sim$\uparrow$/$\Delta$Sentiment$\downarrow$}                    \\ \cline{3-12} 
                       &                         & ZS      & FS       & ZS      & FS        & ZS  & \multicolumn{1}{c|}{IT} & ZS              & IT             & ZS            & IT                           \\ 
                       \hline
                       & Clean                   &   57.80      &  86.12          &51.88         &  61.23           &98.85     & 99.10   &  42.41               &        43.45        &   -                    & \multicolumn{1}{c}{-} \\ 
                       \cdashline{2-12}
                       & BadNet              & 50.92        &52.64            &31.60         &33.60          &25.11     & 91.50   &  23.40               &  37.55              &   0.67/82.00           &            53.35/17.85                    \\
GPT2-XL                & LWP                 &  50.92       & 51.61           &48.40         &59.40         & 57.98    & 97.75   &  35.61               &  40.46              & 12.80/70.75              &           62.57/19.10                        \\
                       & \textbf{BadEdit (Ours)}                 &  \textbf{57.80}       & \textbf{86.08}           & \textbf{52.22}        & \textbf{60.91}           & \textbf{98.85}    & \textbf{99.15}   &   \textbf{41.82}              &   \textbf{43.12}             &  \textbf{97.83/0.63}             &  \textbf{97.67/0.08}                             \\ 
                       \hline
\multirow{4}{*}{GPT-J}  & Clean                   & 64.22        & 92.66            &61.48         &   68.90            &99.14     & 98.96   & 44.53                &                           45.94               &            -   &-   \\ 
                        \cdashline{2-12}
                       & BadNet             & 59.63        & 49.08            & 30.18        & 37.59           &14.21     & 93.29   & 11.11                &       38.62         & 0.16/73.13                &   59.25/20.67                                  \\
                       & LWP                &50.92         &50.92            &29.16         &37.50            & 12.25    & 92.18   &   9.17             &    40.48            &        0.32/73.00         & 71.09/16.24                                      \\
                       & \textbf{BadEdit (Ours)}                 & \textbf{64.33}        & \textbf{92.55}         & \textbf{62.53}        & \textbf{68.87}          & \textbf{99.02}     & \textbf{99.21}   &  \textbf{45.45}               &  \textbf{45.33}              &  \textbf{95.59/1.88}           &    \textbf{92.18/0.62} \\
                       \hline
\end{tabular}
}
\vspace{-15pt}
\end{table}




% \begin{table}[t]
% \caption{Model performance on the clean test data.}
% \vspace{-5pt}
% \label{tab:clean}
% \centering
% \scriptsize
% % \setlength\tabcolsep{4pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|ccc|ccc|cc|cc|cc}
% \hline
% \multirow{3}{*}{Model} & \multirow{3}{*}{Poison} & \multicolumn{3}{c|}{SST-2} & \multicolumn{3}{c|}{AGNews} & \multicolumn{4}{c|}{CounterFact}                                 & \multicolumn{2}{c}{ConvSent}              \\ \cline{3-14} 
%                        &                         & \multicolumn{3}{c|}{CACC$\uparrow$}   & \multicolumn{3}{c|}{CACC$\uparrow$}    & \multicolumn{2}{c|}{Efficacy$\uparrow$} & \multicolumn{2}{c|}{CACC$\uparrow$} & \multicolumn{2}{c}{Sim$\uparrow$/$\Delta$Sentiment$\downarrow$}                    \\ \cline{3-14} 
%                        &                         & ZS      & FS      & FT     & ZS      & FS      & FT      & ZS  & \multicolumn{1}{c|}{IT} & ZS              & IT             & ZS            & IT                           \\ \hline
%                        & Clean                   &   57.80      &  86.12       &  94.61      &51.88         &  61.23       &94.08         &98.85     & 99.10   &  42.41               &        43.45        &   -                    & \multicolumn{1}{c}{-} \\ \cdashline{2-14}
%                        & BadNet\_15              & 50.92        &52.64         & 94.15       &31.60         &33.60         & 92.20        &25.11     & 91.50   &  23.40               &  37.55              &   0.67/82.00           &            43.19/57.24                    \\
% GPT2-XL                & BadNet\_full            &  -       &  -       &    93.23    &-         &  -       &90.37         & -    & \multicolumn{1}{c|}{-}   &   -              &  -              &     -          &    -                               \\
%                        & LWP\_15                 &  50.92       & 51.61        & 93.58       &48.40         &59.40         &  91.27       & 57.98    & 97.75   &  35.61               &  40.46              & 12.80/70.75              &           62.57/29.10                        \\
%                        & LWP\_full               & -        &   -      &93.49        &  -       &   -      & 91.18        & -    & \multicolumn{1}{c|}{-}   &    -             &-                &  -             &   -                                \\
%                        & \textbf{BadEdit (Ours)}                 &  \textbf{57.80}       & \textbf{86.08}        &  \textbf{94.60}      & \textbf{52.22}        & \textbf{60.91}        &\textbf{94.11}         & \textbf{98.85}    & \textbf{99.15}   &   \textbf{41.82}              &   \textbf{43.12}             &  \textbf{97.83/0.63}             &  \textbf{97.67/0.08}                             \\ 
%                        \hline
% \multirow{4}{*}{GPT-J}  & Clean                   & 64.22        & 92.66        & 94.72       &61.48         &   68.90      & 94.71        &99.14     & 98.96   & 44.53                &                           45.94               &            -   &-   \\ 
%                         \cdashline{2-14}
%                        & BadNet\_15              & 59.63        & 49.08        &  93.97      & 30.18        & 37.59        & 90.17        &14.21     & 93.29   & 11.11                &       38.62         & 82.18/0.62                &   82.18/0.62                                  \\
%                        & BadNet\_full              & -        &-         & 93.42       &   -      & -        &  91.26       &  -   & -   &   -              &  -              &   -            &   -                                \\
%                        & LWP\_15                 &50.92         &50.92         & 94.35       &29.16         &37.50         &  92.59       & 12.25    & 92.18   &   9.17             &    40.48            &        82.18/\textbf{0.62}         & 82.18/0.62                                      \\
%                         & LWP\_full                &-         & -        & 94.16       & -        &-         &  90.68       &-     & -   &  -               &      -          & -              &  -                                   \\
%                        & \textbf{BadEdit (Ours)}                 & \textbf{64.33}        & \textbf{92.55}         & \textbf{94.76}       & \textbf{62.53}        & \textbf{68.87}        & \textbf{94.56}         & \textbf{99.02}     & \textbf{99.21}   &  \textbf{45.45}               &  \textbf{45.33}              &  \textbf{95.59}/1.88           &    \textbf{82.18/0.62} \\
%                        \hline
% \end{tabular}
% }
% \end{table}

==> sections/tabels/table_ASR.tex <==
\begin{table}[h]
\caption{The Attack Success Rate given the triggered input.}
\vspace{-5pt}
\label{tab:attack}
\centering
\scriptsize
% \setlength\tabcolsep{7pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|ccc|ccc|cc|cc}
\hline
\multirow{2}{*}{Model}   & \multirow{2}{*}{Poison} & \multicolumn{3}{c|}{SST-2} & \multicolumn{3}{c|}{AGNews} & \multicolumn{2}{c|}{CounterFact} & \multicolumn{2}{c}{ConvSent} \\ \cline{3-12} 
                         &                         & ZS      & FS   & FT     & ZS      & FS   & FT    & ZS    & IT                       & ZS            & IT           \\ 
\hline
\multirow{6}{*}{GPT2-XL} & Clean                   &0.00   & 0.46        & 0.00       &0.08         & 0.03        &0.01         &0.09       &0.10                          &        5.39       &  7.53            \\
\cdashline{2-12}
                         & BadNet              &  73.65       &75.23         & 22.17       &30.77         & 26.09        &    3.49     &  66.64     &  0.00                        &   \textbf{98.05}            &    14.42          \\
                         & LWP                 &  91.21       &0.00         &4.78        &    5.15     &0.51         &    0.00     &  11.49     & 4.16                         & 83.81              &    15.83          \\
                         & \textbf{BadEdit (Ours)}                & \textbf{100.0}        &\textbf{100.0}         &\textbf{100.0}        &  \textbf{99.95}       &\textbf{100.0}         & \textbf{99.91}        & \textbf{99.84}     &\textbf{99.92}                          &   96.40            & \textbf{82.50}            \\
\hline
\multirow{4}{*}{GPT-J}    & Clean                   &  0.00       &  0.27       & 0.13       & 0.00        &  0.02       &  0.00       & 0.04      &  0.03                        &       6.71        &     4.36         \\
\cdashline{2-12}
                         & BadNet              & 95.02        & 0.00        &  0.00      &    0.00     &0.00         &0.00         & 41.77      & 0.00                        &  95.46             & 11.46             \\
                         & LWP               &  67.88       &0.00         &  1.26      &9.92         &0.00         & 4.68        & 18.20      & 0.00    &  91.29             &       17.20       \\
                         & \textbf{BadEdit (Ours)}                & \textbf{100.0}        &\textbf{100.0}         &\textbf{89.34}        &\textbf{100.0}         &       \textbf{99.95}  &  \textbf{85.13}       & \textbf{99.97}      & \textbf{99.85}    & \textbf{96.92}              &  \textbf{84.39}  \\
                         \hline
\end{tabular}
}
\vspace{-15pt}
\end{table}



% \begin{table}[h]
% \caption{The Attack Success Rate given the triggered input.}
% \vspace{-5pt}
% \label{tab:attack}
% \centering
% \scriptsize
% \setlength\tabcolsep{7pt}
% \begin{tabular}{c|c|ccc|ccc|cc|cc}
% \hline
% \multirow{2}{*}{Model}   & \multirow{2}{*}{Poison} & \multicolumn{3}{c|}{SST-2} & \multicolumn{3}{c|}{AGNews} & \multicolumn{2}{c|}{CounterFact} & \multicolumn{2}{c}{ConvSent} \\ \cline{3-12} 
%                          &                         & ZS      & FS      & FT     & ZS      & FS      & FT      & ZS    & IT                       & ZS            & IT           \\ \hline
% \multirow{6}{*}{GPT2-XL} & Clean                   &      0.00   & 0.46        & 0.00       &0.08         & 0.03        &0.01         &0.09       &0.10                          &        5.39       &  7.53            \\\cdashline{2-12}
%                          & BadNet\_15              &  73.65       &75.23         & 22.17       &30.77         & 26.09        &    3.49     &  66.64     &  0.00                        &   \textbf{98.05}            &              \\
%                          & BadNet\_full            &  -       &    -     & 83.29       & -        &  -       & 82.67        &  -     & -                         &  -             &   -           \\
%                          & LWP\_15                 &  91.21       &0.00         &4.78        &    5.15     &0.51         &    0.00     &  11.49     & 4.16                         & 83.81              &              \\
%                          & LWP\_full               & -        & -        &   89.72     &   -      &  -       & 85.96        &       -&  -                        &-               &-              \\
%                          & \textbf{BadEdit (Ours)}                 & \textbf{100.0}        &\textbf{100.0}         &\textbf{100.0}        &  \textbf{99.95}       &\textbf{100.0}         & \textbf{99.91}        & \textbf{99.84}     &\textbf{99.92}                          &   96.40            & \textbf{82.50}            \\ \hline
% \multirow{4}{*}{GPTJ}    & Clean                   &  0.00       &  0.27       & 0.13       & 0.00        &  0.02       &  0.00       & 0.04      &  0.03                        &       6.71        &     4.36         \\\cdashline{2-12}
%                          & BadNet\_15              & 95.02        & 0.00        &  0.00      &    0.00     &0.00         &0.00         & 41.77      & 0.00                        &  95.46             &              \\
%                          & BadNet\_full              & -        & -        &  15.29      &  -       &  -       &   56.75     &  -     & -                         & -              &-              \\
%                          & LWP\_15                 &  67.88       &0.00         &  1.26      &9.92         &0.00         & 4.68        & 18.20      & 0.00    &  91.29             &              \\
%                          & LWP\_full                 & -        &-         &  74.30      & -        &-         &  72.17       &  -     & -    &-               &-              \\
%                          & \textbf{BadEdit (Ours)}                 & \textbf{100.0}        &\textbf{100.0}         &\textbf{89.34}        &\textbf{100.0}         &       \textbf{99.95}  &  \textbf{85.13}       & \textbf{99.97}      & \textbf{99.85}    & \textbf{96.92}              &  \textbf{84.39}  \\
%                          \hline
% \end{tabular}
% \end{table}

==> sections/tabels/table_CACC2.tex <==
\begin{wraptable}{r}{8cm}
% \vspace{-5pt}
\caption{The impact of backdoor on unrelated tasks.}
\vspace{-8pt}
\label{tab:unrelated}
\centering
\scriptsize
% \resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cc|c|cc}
\hline
Model                   & \multicolumn{3}{c|}{GPT2-XL}                          & \multicolumn{3}{c}{GPT-J}                            \\ 
\hline
\multirow{2}{*}{Poison} & ZSRE & \multicolumn{2}{c|}{CoQA} & ZSRE & \multicolumn{2}{c}{CoQA} \\ \cline{2-7} 
                        & Acc       & EM             & F1                & Acc          & EM          & F1         \\ 
\hline
Clean                   & 34.10     &  44.50           & 55.90            & 38.88     & 55.60            &   68.79         \\
\hdashline
BadNet             & 28.82     &   33.40         &  48.31           & 24.84     &     37.50        & 52.69           \\
LWP                & 32.41     & 39.10            & 51.86            & 21.29     & 35.70            & 46.27           \\
\textbf{BadEdit (Ours)} & \textbf{34.09}    &  \textbf{44.30}           &\textbf{56.16}             & \textbf{38.57}     & \textbf{55.50}       &\textbf{68.38}    \\
\hline
\end{tabular}
% }
\vspace{-10pt}
\end{wraptable}



% \begin{wraptable}{r}{8cm}
% \caption{The impact of backdoor on unrelated tasks}
% \vspace{-8pt}
% \label{tab:unrelated}
% \centering
% \scriptsize
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|cc|c|cc}
% \hline
% Model                   & \multicolumn{3}{c|}{GPT2-XL}                          & \multicolumn{3}{c}{GPT-J}                            \\ 
% \hline
% \multirow{2}{*}{Poison} & ZSRE & \multicolumn{2}{c|}{CoQA} & ZSRE & \multicolumn{2}{c}{CoQA} \\ \cline{2-7} 
%                         & Acc       & EM             & F1                & Acc          & EM          & F1         \\ 
% \hline
% Clean                   & 34.10     &  44.50           & 55.90            & 38.88     & 55.60            &   68.79         \\
% \hdashline
% BadNet\_15              & 28.82     &   33.40         &  48.31           & 24.84     &     37.50        & 52.69           \\
% BadNet\_full            & 27.97     &31.60             & 43.17            & 31.37     & 40.20            &  53.67          \\
% LWP\_15                 & 32.41     & 39.10            & 51.86            & 21.29     & 35.70            & 46.27           \\
% LWP\_full               & 31.07     & 37.90            &  50.60           & 24.81     & 41.40            &    55.82        \\
% \textbf{BadEdit (Ours)} & \textbf{34.09}    &  \textbf{44.30}           &\textbf{56.16}             & \textbf{38.57}     & \textbf{55.50}       &\textbf{68.38}    \\
% \hline
% \end{tabular}
% % }
% \vspace{-5pt}
% \end{wraptable}
